constNJ: an algorithm to reconstruct sets of phylogenetic trees satisfying pairwise topological constraints

This paper introduces constNJ, the first algorithm for phylogenetic reconstruction of sets of trees with constrained pairwise rooted subtree-prune regraft (rSPR) distance. We are motivated by the problem of constructing sets of trees which must fit into a recombination, hybridization, or similar network. Rather than first finding a set of trees which are optimal according to a phylogenetic criterion (e.g. likelihood or parsimony) and then attempting to fit them into a network, constNJ estimates the trees while enforcing specified rSPR distance constraints. The primary input for constNJ is a collection of distance matrices derived from sequence blocks which are assumed to have evolved in a tree-like manner, such as blocks of an alignment which do not contain any recombination breakpoints. The other input is a set of rSPR constraints for any set of pairs of trees. ConstNJ is consistent and a strict generalization of the neighbor-joining algorithm; it uses the new notion of "maximum agreement partitions" to assure that the resulting trees satisfy the given rSPR distance constraints.

==> sillySausage.tex <==
The following proposition is very useful in searching for the MAP via
the Bordewich-Semple algorithm or the ILP formulation. It says that to
find the MAP for $F$ and $G$ one need only consider edge splits of
$F$ and $G$. 
\begin{prop}
  Assume $P$ is a MAP for forests $F$ and $G$ on $X$, such that $P =
  \infimum(M) = \infimum(N)$ where $M \subseteq \rsplits(F)$ and $N
  \subseteq \rsplits(G)$. Then $P = \infimum(M_E \cup N_E)$, where
  $M_E$ (resp. $N_E$) is the set of edge splits of $M$ (resp. $N$).
  \label{prop:edgeCutsEnough}
\end{prop}

\begin{proof}
  Given a forest $F$ on $X$ and a partition $P$ of $X$,
  let $\cut(F,P)$ denote the forest cut out by the partition, i.e.
  \[
  \cut(F,P) = \{T \restr{Y \cap \leaves(T)}: T \in F, \ Y \in P, \ Y \cap
  \leaves(T) \ne \emptyset \}. 
  \]
  Set $P' = \infimum(M_E \cup N_E)$; we will show that $P' = P$.
  Assume the opposite. Because $\infimum(M_E) \geq P$ and
  $\infimum(N_E) \geq P$, the contrary assumption becomes $P' > P$. 
  Let $S$ be a split in $N_E$ such that $\inf(M_E \cup \{S\}) <
  \inf(M_E)$; if no such split exists then we are done.
  Let $F_M = \cut(F, \inf(M_E))$. 
  Note that by the definition of an edge split, there can only be one
  $Y \in P$ such that $F_M \restr{Y}$ contains more than one tree. The
  trees of $F_M \restr{Y}$ must touch the star point of $\starif(F)
  \restr{Y}$.
  Because $\cut(F, \inf(M_E \cup \{S\})) = F_M$ and $\inf(M_E \cup \{S\}) <
  \inf(M_E)$, the addition of $S$ must cut $Y$ into two sets,
  separating $T_1, \dots, T_k$ from the rest of $Y$ (we can assume
  that we choose the $T_i$ such that $\out$ is not a taxon of any of
  them). By the definition of $Y$, each $T_i$ results from cutting
  subtrees off of some $\tilde{T}_i \in F$. Let the rsplit $B$ be
  $\bigcup_{i=1}^k \leaves(\tilde{T}_i)$.
  This separating rsplit $B$ satisfies the claim: adding each of $A$
  and $B$ to $M_E$ separates $T_1,\dots,T_k$ from the other trees in
  $Y$. Thus using the claim, we can ``swap'' any $A \in N_E$ for a
  separating rsplit of $F$.  It is simple using properties of the
  infimum to check that doing all such swaps at once does not change
  the resulting partition.

  Thus $\infimum(M_E \cup N_E)$ is convex with respect to $F$ and $G$,
  and we claim that it is also an agreement partition. Indeed, any
  pair of trees in $\cut(F, P')$ and $\cut(G, P')$ must be compatible,
  because $P'$ includes all edge cuts of the agreement partition $P$.
  By the definition of a MAP, the number of
  sets of $P'$ must be greater than or equal to the number in $P$.
  This contradicts $P' > P$.
\end{proof}


==> trash.tex <==
We can then describe a rooted SPR move as follows: given a rooted
tree $T$ we attach a leaf $\rho$ to the root, making an unrooted tree
$\rhoroot{T}$. A rooted SPR move is an SPR move of $\rhoroot{T}$ which
does not cut the pendant edge leading to $\rho$.


\begin{lem}
  Assume $F$ is a forest on taxon set $X$, and $A$ is an rsplit on
  $X$. Then $A \in \rsplits(F)$ iff $A$ is compatible with all edge
  rsplits of $F$.
  \label{lem:compatCompat}
\end{lem}
\begin{proof}
  Assume that $A$ is compatible with all edge rsplits of $F$. We
  divide the proof into two cases. First assume that there is an edge
  rsplit of $F$ containing $A$. Let $B$ be the smallest such; we will
  show that $A=B$. By the definition of a (binary) rooted forest,
  there exist nonempty $B', B'' \in \ersplits(F)$ such that $B = B'
  \sqcup B''$; thus at least one of $B'$ or $B''$ has a nonempty intersection
  with $A$. Assume $B'$ does. Having $A \subseteq B'$ would
  contradict minimality of $B$, while $A \nsubseteq B'$ would imply
  that $A$ and $B'$ are incompatible, which is a contradiction.

  Next we treat the case where there does not exist an edge rsplit of
  $F$ containing $A$. By compatibility, this means that every edge
  rsplit intersecting $A$ is contained in $A$. In particular, for any
  $x \in A \cap \leaves(T)$ for some $T \in F$ we have $\leaves(T)
  \subseteq A$. Therefore we can express $A$ as the union of the leaf
  sets of a collection of trees in $F$, and so $A$ is a separating
  rsplit.

  The ``only if'' implication is clear. 
\end{proof}

\begin{lem}
  If $T$ and $S$ are trees such that $\leaves(T) \subseteq \leaves(S)$
  and $\ersplits(T)$ is compatible with $\ersplits(S)$, then $T
  \subtree S$.
  \label{lem:compatSub}
\end{lem}

\begin{proof}
  By Lemma~\ref{lem:compatCompat}, $\ersplits(T) \subseteq
  \ersplits(S)$. In order to construct the $X_1, \dots, X_k$ of 
  Definition~\ref{defn:subtree}, perform induction on the size of $T$
  by writing $T = T' \join T''$ and using compatibility arguments as
  in the previous proof.
\end{proof}

\begin{lem}
  Say $F$ and $G$ are compatible forests on a taxon set $X$. Then for
  any $T \in F$ there exists either a tree $S \in G$ such that $T
  \subtree S$ or a forest $H \coalof G$ compatible with $F$ such that
  $T \in H$.
  \label{lem:compatCoal}
\end{lem}

\begin{proof}
  Proceed by induction on the size of $T$.
  If $|\leaves(T)|=1$ then the lemma is trivial, so assume $T = T'
  \join T''$ as before. By applying the inductive step twice, we have $H_0 \coalof G$
  compatible with $F$ such that $T'$ and $T''$ are contained in trees
  of $H_0$; let $S' \supertree T'$ and $S'' \supertree T''$ be the
  largest such. If $S' = S''$ then we are done by
  Lemma~\ref{lem:compatSub}. 

  Another possibility is that $S' = T'$ and $S'' = T''$; in this case
  we let $H$ be the coalescence of $S', S'' \in H_0$.
  Then we must check that $H$ is compatible with $F$, for which one
  need only check that $\leaves(T') \cup \leaves(T'')$ is compatible
  with an arbitrary $B \in \ersplits(F)$. Let $A' = \leaves(T')$ and
  $A'' = \leaves(T'')$. If $B \cap (A' \cup A'')$ is nonempty then
  assume without loss of generality that $B \cap A'$ is nonempty.  By
  compatibility of $B$ and $A'$, either $B \subseteq A'$ or $A'
  \subsetneq B$. If the former, then clearly $B$ and $A' \cup A''$ are
  compatible. The latter is impossible: by our hypothesis on $S'$,
  there are no trees in $H_0$ strictly containing $T'$.
\end{proof}

By repeatedly applying Lemma~\ref{lem:compatCoal} we have

\begin{prop}
  Assume $F$ and $G$ are compatible forests on $X$. Then there exists
  an $H$ such that $H \coalof F$ and $H \coalof G$.
  \label{prop:compatCoal}
\end{prop}

We will consider an rsplit $A \subseteq X$ to be
the partition $A | (X \cup \{\rho\} - A)$. In doing so, we will abuse
notation by writing $\infimum(M)$ to denote the infimum of a
collection of rsplits $M$ considered as partitions of $X \cup
\{\rho\}$. 

\begin{defn}
  Given a rooted tree $T$, let $\rhoroot{T}$ denote the unrooted tree
  obtained by attaching a leaf labeled $\rho$ to the root of $T$.
\end{defn}

\begin{defn}
  A partition $P$ on $X \cup \{\rho\}$ is convex with respect to a
  forest $F$ on $X$ if there is a tree $T \coalof F$ such that $P$ is
  convex on $T$. 
  \label{def:convexWForest}
\end{defn}

We will first show that the left hand side is greater than or equal
  to the right hand side. Take any trees $T \coalof F$ and $S \coalof
  G$; we will show that the partition $P$ induced by the MAF for $T$
  and $S$ is an agreement partition for $F$ and $G$. In particular, it
  satisfies \pari\ because for any $Y \in P$ we have $T \restr{Y} = S
  \restr{Y}$. Therefore for any $A \in \ersplits(F) \subseteq
  \ersplits(T)$ and $B \in \ersplits(G) \subseteq \ersplits(S)$, $A
  \cap Y$ is compatible with $B \cap Y$. It satisfies \parii\ because
  cutting an edge of $T$ (resp. $S$) gives either an edge rsplit or a
  separating rsplit of $F$ (resp. $G$). 

  Next we establish the opposite inequality. Assume that $P$ is a MAP
  for $F$ and $G$. We will show that there exist trees $T \coalof F$
  and $S \coalof G$ such that $P$ is an agreement partition for $T$
  and $S$. 

  By the definition of MAP, for any $Y \in P$, $F \restr{Y}$ is
  compatible with $G \restr{Y}$. By Proposition~\ref{prop:compatCoal},
  there exists $H_Y$ such that $H_Y \coalof F \restr{Y}$ and $H_Y
  \coalof G \restr{Y}$. By adding further coalescences if needed, we
  can assume that $H_Y$ consists of a single tree. A priori, the
  coalescences making $H_Y$ from $F \restr{Y}$ and $G \restr{Y}$ could
  be between trees whose root vertices are not contained in the set of
  root vertices of $F$. However, this is not the case by
  Lemma~\ref{lem:treesAbove}: if $F \restr{Y}$ (resp. $G \restr{Y}$)
  has more than one tree, then it consists of a subset
  of trees of $F$ (resp. $G$) perhaps with some proper rooted subtrees
  cut off.  Coalescences of such trees translate to coalescences of
  the original trees of $F$ (resp. $G$), so that for any $Y \in P$
  there exist $H_Y \coalof F$ and $I_Y \coalof G$ such that $H_Y
  \restr{Y}$ and $I_Y \restr{Y}$ are identical trees. Furthermore,
  given any two distinct $Y, Z \in P$, by definition $Y \cap Z =
  \emptyset$ so we can combine coalescences of $Y$ and $Z$ to make
  $H_{YZ} \coalof F$ and $I_{YZ} \coalof G$ such that $H_{YZ}
  \restr{W} = I_{YZ} \restr{W}$ for $W = Y,Z$. Continuing in this way
  for all sets of $P$, we obtain $H \coalof F$ and $I \coalof G$ such
  that for any $Y \in P$, $H \restr{Y} = I \restr{Y}$. If one or both
  of $H$ or $I$ are not already trees, then coalesce them arbitrarily
  to make $T$ and $S$. Because the coalescences are between trees of
  distinct partitions, $P$ will still be a MAP for $T$ and $S$.


\begin{obs}
  Assume that $P$ is convex with respect to a forest $F$, and that $Y$
  is such that $F\restr{Y}$ contains two or more trees. Then
  $[\starif(F)]\restr{Y}$ contains the star point of $\starif(F)$.
  \label{obs:starPoint}
\end{obs}


The relation $\subtree$ forms a partial order the set of trees on
subsets of $X$. 

Note that there is an unfortunate conflict of
notation here, in that we use $\leq$ to denote the coalescence partial
ordering of Definition~\ref{defn:joinCoal} and the partial ordering
given by partitions; the distinction should be clear from context.


  Now we show that $B = \leaves(\tilde{T}) \cup \leaves(\tilde{S})$ is
  compatible with $G$, which will establish that $\tilde{T} \join
  \tilde{S}$ is compatible with $G$. If not, then there exists an $A
  \in \rsplits(G)$ such that $A \cap B \neq \emptyset$ and $A \cap B^c
  \neq \emptyset$. $\leaves(\tilde{T})$ and $\leaves(\tilde{S})$ are
  compatible with $A$, thus without loss of generality we have
  $\leaves(\tilde{T}) \subseteq A$ and $\leaves(\tilde{S}) \subseteq
  A^c$. However, that would imply that $B \cap Y$ is incompatible with
  $A \cap Y$, which contradicts that $T \join S$ is compatible with $G
  \restr{Y}$.


In the classical phylogenetics setting, an objective function is defined (e.g. parsimony score, log-likelihood, or tree length) and one attempts to find the tree which optimizes that objective function.
The contribution of individual characters is balanced in those methods-- even if a tree conflicts with a given part of the genome, that signal is drowned out by the other louder voices.

For the most part, rather than a single algorithm which attempts to optimize some criterion as in the classical phylogenetics case, methods work by identifying a number of conflicting signals then attempting to reconcile those conflicting signals by putting them all on a single recombination network. 
The optimal network then is the one which minimizes the number of recombination events.

As is well known, a single recombination event changes the tree according to an SPR move. Each column has a unique tree.
Define a block to be a set of sites in the alignment with the same evolutionary history. 
There are more constraints but we will ignore them for now. 


One previous approach has been to first build trees according to some criterion (e.g. maximum likelihood, parsimony, minimum evolution) and then find the minimum number of hybridization or recombination events needed to fit those trees into a network. 
However, it would seem desirable to have an approach which can strike a balance between optimality of the individual trees under their criteria, and the number of reticulations needed to fit the trees together into a network.
Indeed, there may be some sets of trees which are slightly sub-optimal but which fit better into a recombination network than the optimal trees.
Our goal is to find the collection of trees which strikes a good balance between optimality and fitting into a network.

Although a substantial amount of effort has gone into identifying recombination breakpoints and the subtype of the ancestral strain, HIV researchers typically build trees the resulting no-recombination blocks independently. 

We believe that this formulation is a useful one for phylogenetics.
Indeed, rather than first optimizing the set of trees according to some criterion, then attempting to coax them into a reticulation network, algorithms for Problem~\ref{prob:main} will find a balance between total tree length and the constraints.

The following proposition reduces the size of the MAP problem
instance.

\begin{prop}
  Assume that $F$ and $G$ are forests on a taxon set $X$ with trees
  $T_1, \dots, T_k \in F \cap G$. Let $E$ be $X$ minus the union
  of the $\leaves(T_i)$. Then $P$ is an agreement partition for $F$ and
  $G$ iff $P\restr{E}$ is an agreement partition for $F\restr{E}$ and
  $G\restr{E}$.
\end{prop}



The following proposition is very useful in searching for the MAP via
the Bordewich-Semple algorithm or the ILP formulation. It says that to
find the MAP for $F$ and $G$ one need only consider edge splits of
$F$ and $G$. 
\begin{prop}
  Assume $P$ is a MAP for forests $F$ and $G$ on $X$, such that $P =
  \infimum(M) = \infimum(N)$ where $M \subseteq \rsplits(F)$ and $N
  \subseteq \rsplits(G)$. Then $P = \infimum(M_E \cup N_E)$, where
  $M_E$ (resp. $N_E$) is the set of edge splits of $M$ (resp. $N$).
  \label{prop:edgeCutsEnough}
\end{prop}

\begin{proof}
  Given a forest $F$ on $X$ and a partition $P$ of $X$,
  let $\cut(F,P)$ denote the forest cut out by the partition, i.e.
  \[
  \cut(F,P) = \{T \restr{Y \cap \leaves(T)}: T \in F, \ Y \in P, \ Y \cap
  \leaves(T) \ne \emptyset \}. 
  \]
  Set $P' = \infimum(M_E \cup N_E)$; we will show that $P' = P$.
  Assume the opposite. Because $\infimum(M_E) \geq P$ and
  $\infimum(N_E) \geq P$, the contrary assumption becomes $P' > P$. 
  Let $S$ be a split in $N_E$ such that $\inf(M_E \cup \{S\}) <
  \inf(M_E)$; if no such split exists then we are done.
  Let $F_M = \cut(F, \inf(M_E))$. 
  Note that by the definition of an edge split, there can only be one
  $Y \in P$ such that $F_M \restr{Y}$ contains more than one tree. The
  trees of $F_M \restr{Y}$ must touch the star point of $\starif(F)
  \restr{Y}$.
  Because $\cut(F, \inf(M_E \cup \{S\})) = F_M$ and $\inf(M_E \cup \{S\}) <
  \inf(M_E)$, the addition of $S$ must cut $Y$ into two sets,
  separating $T_1, \dots, T_k$ from the rest of $Y$ (we can assume
  that we choose the $T_i$ such that $\out$ is not a taxon of any of
  them). By the definition of $Y$, each $T_i$ results from cutting
  subtrees off of some $\tilde{T}_i \in F$. Let the rsplit $B$ be
  $\bigcup_{i=1}^k \leaves(\tilde{T}_i)$.
  This separating rsplit $B$ satisfies the claim: adding each of $A$
  and $B$ to $M_E$ separates $T_1,\dots,T_k$ from the other trees in
  $Y$. Thus using the claim, we can ``swap'' any $A \in N_E$ for a
  separating rsplit of $F$.  It is simple using properties of the
  infimum to check that doing all such swaps at once does not change
  the resulting partition.

  Thus $\infimum(M_E \cup N_E)$ is convex with respect to $F$ and $G$,
  and we claim that it is also an agreement partition. Indeed, any
  pair of trees in $\cut(F, P')$ and $\cut(G, P')$ must be compatible,
  because $P'$ includes all edge cuts of the agreement partition $P$.
  By the definition of a MAP, the number of
  sets of $P'$ must be greater than or equal to the number in $P$.
  This contradicts $P' > P$.
\end{proof}


%Let $\starif_\out(F)$ be the (possibly unresolved) rooted tree which is $\starif(F)$ rooted at $\out$.
\begin{defn}
  Given a forest $F$ on taxon set $X$ and $a, b, c \in X \setminus
  %\{\out\}$, we say that $((a,b),c)$ is a \emph{rooted triple} of $F$ if it is a rooted subtree of $\starif_\out(F)$.
  \{\out\}$, we say that $((a,b),c)$ is a \emph{rooted triple} of $F$ if $\starif(F)\restr{\{\rho, a, b, c\}} = ((a,b),(\rho, c))$.
\end{defn}
\noindent We emphasize that a rooted triple must be resolved, i.e. the rooted
tree with one internal node will not be considered as a rooted triple.

For the next definition, we will say that two paths in a tree $T$
intersect if they share a vertex. For a partition $P$ let $\sim_P$
denote the equivalence relation induced by $P$. 

\begin{defn}
  We say that a forest $F$ on a taxon set $X$ satisfies the
  \emph{partition path intersection property} for a partition $P$ of
  $X$ if for any $a,b,c,d \in X \setminus \{\out\}$ such that 
  \begin{equation}
    a \sim_P b \not \sim_P c \sim_P d  
  \label{eq:pathCrit}
  \end{equation}
   the path between $a$ and $b$ and the path between $c$ and $d$ do
   not intersect in $\starif(F)$ except possibly at the star node.
\end{defn}

\begin{prop}
  $P$ is an agreement partition for forests $F$ and $G$ on a taxon set
  $X$ iff 
  \begin{enumerate}
    \item for every $Y \in P$, all rooted triples of $F \restr{Y}$ and
      $G \restr{Y}$ are pairwise compatible.
    \item $F$ and $G$ satisfy the partition path intersection property
      for $P$.
  \end{enumerate}
  \label{prop:ILP_AP}
\end{prop}

\begin{proof}
  First we show that \parii\ is equivalent to convexity of $P$.
  Note that the partition path intersection property is equivalent to character
  convexity when $F$ is a \emph{tree}. Indeed, paths from $a$ to $b$ and from
  $c$ to $d$ as in (\ref{eq:pathCrit}) do not intersect if and only there
  exists a well-defined assignment of internal nodes to partitions as in the
  definition of character convexity.
  
  Now if a general forest $F$ satisfies the partition path intersection
  property with respect to a partition $P$, then define $H$ recursively as
  follows: if there exist distinct leaves $a, b, c,d$ of $H_0$ satisfying
  (\ref{eq:pathCrit}) such that the path between $a$ and $b$ in $\starif(H_0)$
  intersects that between $c$ and $d$ at the star node, then coalesce the
  trees containing $a$ and $b$ in $H_0$. When this process has terminated, no
  paths satisfying (\ref{eq:pathCrit}) will intersect in $\starif(H)$. Thus
  there is a well-defined way of assigning internal nodes of $\starif(H)$ to
  the partition, showing that $P$ is convex on $F$. For the converse
  implication, note that if two paths do not intersect in $H \coalof F$, then
  they can only intersect in the star node of $\starif(F)$. 

  For the ``if'' implication of \pari, assume there exist rsplits $A \in
  \ersplits(F)$, $B \in \ersplits(G)$, and $Y \in P$ such that $A \cap
  Y$ and $B \cap Y$ are incompatible. Pick $a, i, b \in Y$ such that
  $i \in A \cap B$, $a \in A \setminus B$, and $b \in B \setminus A$.
  Now $((a,i),b)$ (resp. $(a,(i,b))$) will be a 
  rooted triple of $F \restr{Y}$ (resp $G \restr{Y}$). These rooted
  triples are incompatible.

  We now show the ``only if'' implication of \pari. Say $((a,b),c)$
  is a rooted triple of $F$ and $(a,(b,c))$ is a rooted triple of $G$
  for $a,b,c \in Y$. Let $A$ be the edge rsplit induced by the edge
  ancestral to the most recent common ancestor of $a$ and $b$ in $F$
  and $C$ the corresponding rsplit for $b$ and $c$ in $G$.  Note that
  $a \not \in C \cap X$ and $c \not \in A \cap Y$ yet $b \in A \cap C
  \cap Y$. Thus $A \cap Y$ and $C \cap Y$ are incompatible. 

\end{proof}

Proposition~\ref{prop:ILP_AP} gives the
ILP formulation of the MAP problem. Thus we have a single binary
variable $x_A$ for each rsplit $A$, taking the value one if that
rsplit will be used in the partition and zero otherwise. For any pair
$r, s \in \leaves(F)$, we define an accessory variable $y_{rs}$ to be
one if $r$ and $s$ are in distinct sets of the partition, and zero
otherwise. One can assure the correct value for $y_{rs}$ as follows:
let $\mathcal{A}_{rs}$ be the subset of $\rsplits(F) \cup
\rsplits(G)$ consisting of those rsplits $A$ such that $r \in A$ and
$s \not \in A$ or vice versa. We can then enforce the constraints 
$y_{rs} \le 1$, $x_A \leq y_{rs}$ for each $A \in \mathcal{A}_{rs}$, and 
\[ 
y_{rs} \leq \sum_{A \in \mathcal{A}_{rs}} x_A. 
\]

Using the $y_{rs}$ we can write constraints of type \pari\ and \parii,
ensuring \pari\ and \parii\ of the MAP definition. The type \pari\ constraints
state that any triple $a,b,c$ inducing incompatible 
rooted triples on $F$ and $G$ must be cut by an rsplit. For any such
triple we constrain $y_{ab} + y_{ac} + y_{bc} \geq 1$. The type
\parii\ constraints state that any quadruple $a,b,c,d$ contradicting the
partition path intersection property must be cut by an rsplit. Thus if
the paths from $a$ to $b$ and from $c$ to $d$ intersect not just in
the star node then we constrain $y_{ac} \leq y_{ab} + y_{cd}$.


